Dynamical behavior of Predator-Prey with Allee Effect on Both Populations and Disease in Predator

In the current study, we took into account a model of nonlinear ``predator-prey'' interactions including the ``Allee effect'' on both populations and disease in the predator population. The population as a whole is split into three: the prey population, susceptible predator, and diseased predator. The ``Takagi-Sugeno (T-S) impulsive control model'' and the Fuzzy impulsive control model have been used to test the stability of the three-dimensional ``Lotka-Volterra predator-prey system'' model. Following the model's formulation, the global-stability and the fuzzy solution are examined using numerical simulations and graphical displays, together with the necessary consultation, to help comprehend the effectiveness of our suggested model.

==> Makefile <==
#
# Makefile for aomart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.7 2017/12/14 03:25:19 boris Exp $
#

PACKAGE=aomart

SAMPLES = \
	aomsample.tex\
	aomsample1.tex \
	aomfrench.tex

PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

aomsample1.tex: fullref.pl aomsample.tex
	perl fullref.pl aomsample.tex > aomsample1.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) aomsample1.tex

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1  \
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' \
	--exclude '*.tgz' --exclude '*.zip'  --exclude CVS $(PACKAGE)
	mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> README <==
	      LaTeX Class for The Annals of Mathematics
			    Boris Veytsman
			    Version 1.27

This package provides the class for typesetting articles for The Annals
of Mathematics, http://annals.princeton.edu/.  

Changes:

    Version 1.27
    	 New command: \funding

    Version 1.26
          Interface for contributors

    Version 1.25
          New command: \fullpageref

    Version 1.24
          Optionally print MSC designation

    Version 1.23
          Large ymath symbols are now default

    Version 1.22
          Changed margins for screen mode

    Version 1.21
          Better support of internationalization

    Version 1.20
    	  Print primary and secondary subjects separately
	  We no longer print url if doi is present

    Version 1.19
          Bibliography changes

    Version 1.18
    	  Now we print keywords and AMS subjects
	  Added orcid

    Version 1.17a
          Bug fixed in aomplain.bst

    Version 1.17
          New field totalpages in the bibliography

    Version 1.16
          Metadata handling changes. 

    Version 1.15
          New doi formatting

    Version 1.14a
          New url on the masthead

    Version 1.14
          Added macros for Crossref submissions

    Version 1.13
          The correction in v1.12 did not work with older hyperref
          versions.  This release corrects the problem.

    Version 1.12
          Corrected the bug with hyperref and appendix

    Version 1.11
          Added \copyrightnote
          Added \fulladdress
          Bibliography changes: added titlenote field, 
                                deleted \bysame line
          Bug fix with e-mail including underscores
    
    Version 1.10
          `Old' doi formatting can be set with the option olddoi
          Support for French and German added

    Version 1.9
          Changed formatting of doi numbers

    Version 1.8
          Bibliography changes: 
            @incollection now the uses venue field;
            "von" part is not used when ordering entries.

    Version 1.7
          Suppressed end page number in the header for one-page 
            documents

    Version 1.6
          Appendix letter is now upright in the refs, even inside
            italics
          Bibliography style change: aomalpha.bst now respects the 
            key field

    Version 1.5
           Typo corrected: arXiV is now arXiv
           Bibliography style change: added sortyear field

    Version 1.4
           Changed formatting of sections and subsections

    Version 1.3  
           Bug fixes
           Bibliography style change:  added url field

